Automatic Anomaly Detection in the Cloud Via Statistical Learning

Performance and high availability have become increasingly important drivers, amongst other drivers, for user retention in the context of web services such as social networks, and web search. Exogenic and/or endogenic factors often give rise to anomalies, making it very challenging to maintain high availability, while also delivering high performance. Given that service-oriented architectures (SOA) typically have a large number of services, with each service having a large set of metrics, automatic detection of anomalies is non-trivial. Although there exists a large body of prior research in anomaly detection, existing techniques are not applicable in the context of social network data, owing to the inherent seasonal and trend components in the time series data. To this end, we developed two novel statistical techniques for automatically detecting anomalies in cloud infrastructure data. Specifically, the techniques employ statistical learning to detect anomalies in both application, and system metrics. Seasonal decomposition is employed to filter the trend and seasonal components of the time series, followed by the use of robust statistical metrics -- median and median absolute deviation (MAD) -- to accurately detect anomalies, even in the presence of seasonal spikes. We demonstrate the efficacy of the proposed techniques from three different perspectives, viz., capacity planning, user behavior, and supervised learning. In particular, we used production data for evaluation, and we report Precision, Recall, and F-measure in each case.

==> data.tex <==
\subsubsection{Data Collection} \label{sec:data}

The efficacy of S-ESD and S-H-ESD was analyzed over a wide corpus of time series
data obtained from \textit{production}. In the current context, i.e., at
Twitter, and for other social networks, it was important to cover both low-level
\textit{system metrics} and higher level \textit{core drivers} (business
metrics). To this end, the following metrics were used:

\begin{dinglist}{114} 
\item System Metrics 
\begin{dinglist}{114}
  \item CPU utilization 
  \item Disk writes
\end{dinglist}
\item Core Drivers 
\begin{dinglist}{114} 
  \item Tweets per minute (TPM) 
  \item Retweets per minute (RTPM) 
  \item Unique Photos Per Minute (UPPM) 
\end{dinglist}
\end{dinglist}

In total, 20 data sets were investigated which included 10 system metrics and 10
core drivers. The system metrics ranged from two-week long periods to four-week
long periods, with hourly granularity. The core drivers metrics were all
minutely data over four-week periods.


==> s-esd-algo_backup.tex <==
We now present a formal description of S-ESD. 

\begin{algorithm}[h]
\begin{algorithmic}
\STATE \ \
\STATE {\bf Input}: Raw time series \\[1mm]
\STATE {\bf Output:} FILL IN \\[2mm]
\STATE FILL IN \\[1mm] 
\STATE Eliminate redundant {\tt wait}s \\[1mm]
\STATE Let {\bf U} = {\tt post} FILL IN \\[1mm]
\STATE /* Some Comment  */ \\[1mm]
\FOR{{\bf each} operation {\em op} in {\bf U}}
  \IF{{\em op} is a conditional}
    \STATE DO SOMETHING 
  \ELSE
    \STATE DO SOMETHING ELSE
  \ENDIF
\ENDFOR
\STATE \ \
\STATE Let {\bf D} = {\tt wait}s 
\STATE /* Comment  */ \\[1mm]
\FOR{{\bf each} operation {\em op} in {\bf D}}
  \IF{{\em op} is not a conditional}
    \STATE BLAH 
  \ENDIF
\ENDFOR
\end{algorithmic}
\caption{S-ESD Algorithm}
\label{algo:s}
\end{algorithm}

\noindent First, \algoref{algo:alg} renames BLAH. Subsequently, it 


==> s-h-esd-algo.tex <==
We now present a formal description of S-H-ESD. 

\begin{algorithm}[h]
\begin{algorithmic}
\STATE \ \
\STATE {\bf Input}: \\[1mm]
 	$Y_t$ = A time series \\[1mm]
 	$n$ = number of obs. in $Y_t$ \\[1mm]
 	$k$ = max anomalies \\
\bigskip
\STATE {\bf Output:} \\[1mm]
 	$v$ = A time-stamped anomaly vector
\bigskip
\STATE {\bf Require:} \\[1mm]
 		$k \leq (n \times .49)$ \\[1mm]
\STATE 1. Follow steps 1-3 from \algoref{algo:s-esd-algo} \\[1mm] 
\STATE 2. Run ESD on $R_t$ using the $\tilde{Y}$ and $MAD$ in the calculation of the test statistic\\
\bigskip
\RETURN $v = R_t \cap Y_t$

\end{algorithmic}
\caption{S-H-ESD Algorithm}
\label{algo:s-h-esd-algo}
\end{algorithm}


==> sesd-shesd-cap-ub-fmeasure-table.tex <==
\begin{table*}[ht]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{|c|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\textit{One-Tail (Capacity)}                      & \multicolumn{6}{|c|}{\textit{Alpha = 0.05}}                                                                                                                                                                                                             & \multicolumn{6}{|c|}{\textit{Alpha = 0.001}}                                                                                                                                                                                                            & \multicolumn{1}{|c|}{\# of Observations} \\ \hline
\multicolumn{1}{|l|}{}                            & \multicolumn{3}{|c|}{\textbf{S-ESD}}                                                                                       & \multicolumn{3}{|c|}{\textbf{S-H-ESD}}                                                                                     & \multicolumn{3}{|c|}{\textbf{S-ESD}}                                                                                       & \multicolumn{3}{|c|}{\textbf{S-H-ESD}}                                                                                     &                                          \\ \hline
\textbf{Dataset \#}                       & \textit{Precision}                       & \textit{Recall}                       & \textit{Fmeasure}                       & \textit{Precision}                       & \textit{Recall}                       & \textit{Fmeasure}                       & \textit{Precision}                       & \textit{Recall}                       & \textit{Fmeasure}                       & \textit{Precision}                       & \textit{Recall}                       & \textit{Fmeasure}                       &                                          \\ \hline
System 1                                  & 1.00                                     & 0.05                                  & 0.09                                    & 0.26                                     & 1.00                                  & 0.41                                    & 1.00                                     & 0.02                                  & 0.05                                    & 0.28                                     & 1.00                                  & 0.44                                    & 337                                      \\ \hline
System 2									 & 1.00                                     & 0.04                                  & 0.07                                    & 0.95                                     & 0.87                                  & 0.91                                    & 1.00                                     & 0.00                                  & 0.01                                    & 0.95                                     & 0.81                                  & 0.88                                    & 721                                      \\ \hline
System 3									 & 1.00                                     & 0.14                                  & 0.25                                    & 0.98                                     & 0.93                                  & 0.95                                    & 1.00                                     & 0.01                                  & 0.01                                    & 1.00                                     & 0.77                                  & 0.87                                    & 601                                      \\ \hline
System 4									 & 1.00                                     & 0.57                                  & 0.73                                    & 0.71                                     & 0.99                                  & 0.82                                    & 1.00                                     & 0.43                                  & 0.60                                    & 0.84                                     & 0.95                                  & 0.89                                    & 913                                      \\ \hline
System 5									 & 0.98                                     & 1.00                                  & 0.99                                    & 0.98                                     & 1.00                                  & 0.99                                    & 0.98                                     & 1.00                                  & 0.99                                    & 0.98                                     & 1.00                                  & 0.99                                    & 337                                      \\ \hline
System 6									 & 0.75                                     & 0.28                                  & 0.41                                    & 0.65                                     & 0.34                                  & 0.45                                    & 0.80                                     & 0.13                                  & 0.22                                    & 0.75                                     & 0.28                                  & 0.41                                    & 721                                      \\ \hline
\multicolumn{1}{|c|}{\textbf{AVERAGES}}   & \BlackCell{0.96}                         & \BlackCell{0.35}                          & \BlackCell{0.42}                        & \BlackCell{0.75} 						   & \BlackCell{0.85}                                  & \BlackCell{0.76}                      	 & \BlackCell{0.96}                         & \BlackCell{0.26}                                  & \BlackCell{0.31}                        & \BlackCell{0.80}                         & \BlackCell{0.80}                                  & \BlackCell{0.75}                        &                                          \\ \hline
Core Driver 1                             & 0.99                                     & 0.48                                  & 0.65                                    & 0.83                                     & 0.78                                  & 0.80                                    & 1.00                                     & 0.40                                  & 0.57                                    & 0.95                                     & 0.61                                  & 0.74                                    & 43195                                    \\ \hline
Core Driver 2                             & 1.00                                     & 0.03                                  & 0.06                                    & 0.96                                     & 0.25                                  & 0.39                                    & 1.00                                     & 0.01                                  & 0.02                                    & 1.00                                     & 0.05                                  & 0.10                                    & 43200                                    \\ \hline
Core Driver 3                             & 0.08                                     & 1.00                                  & 0.14                                    & 0.05                                     & 1.00                                  & 0.10                                    & 0.12                                     & 1.00                                  & 0.22                                    & 0.08                                     & 1.00                                  & 0.14                                    & 43200                                    \\ \hline
Core Driver 4                             & 0.34                                     & 0.20                                  & 0.25                                    & 0.20                                     & 0.30                                  & 0.24                                    & 0.54                                     & 0.18                                  & 0.27                                    & 0.29                                     & 0.22                                  & 0.25                                    & 43200                                    \\ \hline
Core Driver 5                             & 0.36                                     & 0.98                                  & 0.52                                    & 0.19                                     & 0.98                                  & 0.32                                    & 0.53                                     & 0.98                                  & 0.69                                    & 0.33                                     & 0.98                                  & 0.49                                    & 43200                                    \\ \hline
Core Driver 6                             & 0.08                                     & 0.69                                  & 0.14                                    & 0.06                                     & 0.69                                  & 0.11                                    & 0.12                                     & 0.69                                  & 0.20                                    & 0.08                                     & 0.69                                  & 0.14                                    & 43200                                    \\ \hline
Core Driver 7                             & 0.27                                     & 0.97                                  & 0.42                                    & 0.20                                     & 0.97                                  & 0.33                                    & 0.33                                     & 0.97                                  & 0.49                                    & 0.25                                     & 0.97                                  & 0.40                                    & 43200                                    \\ \hline
Core Driver 8                             & 0.66                                     & 0.95                                  & 0.78                                    & 0.58                                     & 0.99                                  & 0.73                                    & 0.80                                     & 0.63                                  & 0.71                                    & 0.67                                     & 0.95                                  & 0.78                                    & 43200                                    \\ \hline
Core Driver 9                             & 0.80                                     & 0.54                                  & 0.65                                    & 0.58                                     & 0.63                                  & 0.60                                    & 0.91                                     & 0.53                                  & 0.67                                    & 0.72                                     & 0.56                                  & 0.63                                    & 43178                                    \\ \hline
Core Driver 10                            & 0.82                                     & 0.20                                  & 0.32                                    & 0.67                                     & 0.30                                  & 0.42                                    & 1.00                                     & 0.08                                  & 0.14                                    & 0.81                                     & 0.20                                  & 0.32                                    & 43200                                    \\ \hline
\multicolumn{1}{|c|}{\textbf{AVERAGES}}   & \BlackCell{0.54}                         & \BlackCell{0.60}                                  & \BlackCell{0.39}                        & \BlackCell{0.43}                         & \BlackCell{0.69}                                  & \BlackCell{0.40}                        & \BlackCell{0.63}                         & \BlackCell{0.55}                          & \BlackCell{0.40}                        & \BlackCell{0.52}                         & \BlackCell{0.62}                                  & \BlackCell{0.40}                        &                                          \\ \hline
One-Tail (User Behavior)                  & \multicolumn{6}{|c|}{\textit{Alpha = 0.05}}                                                                                                                                                                                                             & \multicolumn{6}{|c|}{\textit{Alpha = 0.001}}                                                                                                                                                                                                            & \multicolumn{1}{|c|}{\# of Observations} \\ \hline
\multicolumn{1}{|l|}{}                    & \multicolumn{3}{|c|}{\textbf{S-ESD}}                                                                                       & \multicolumn{3}{|c|}{\textbf{S-H-ESD}}                                                                                     & \multicolumn{3}{|c|}{\textbf{S-ESD}}                                                                                       & \multicolumn{3}{|c|}{\textbf{S-H-ESD}}                                                                                     &                                          \\ \hline
\textbf{Dataset \#}                               & \multicolumn{1}{|c|}{\textit{Precision}} & \multicolumn{1}{|c|}{\textit{Recall}} & \multicolumn{1}{|c|}{\textit{Fmeasure}} & \multicolumn{1}{|c|}{\textit{Precision}} & \multicolumn{1}{|c|}{\textit{Recall}} & \multicolumn{1}{|c|}{\textit{Fmeasure}} & \multicolumn{1}{|c|}{\textit{Precision}} & \multicolumn{1}{|c|}{\textit{Recall}} & \multicolumn{1}{|c|}{\textit{Fmeasure}} & \multicolumn{1}{|c|}{\textit{Precision}} & \multicolumn{1}{|c|}{\textit{Recall}} & \multicolumn{1}{|c|}{\textit{Fmeasure}} &                                          \\ \hline
System 1                                  & 1.00                                     & 0.02                                  & 0.04                                    & 0.60                                     & 1.00                                  & 0.75                                    & 1.00                                     & 0.01                                  & 0.02                                    & 0.65                                     & 1.00                                  & 0.79                                    & 337                                      \\ \hline
System 2                                  & 1.00                                     & 0.03                                  & 0.06                                    & 1.00                                     & 0.68                                  & 0.81                                    & 1.00                                     & 0.00                                  & 0.01                                    & 1.00                                     & 0.63                                  & 0.77                                    & 721                                      \\ \hline
System 3                                  & 1.00                                     & 0.12                                  & 0.22                                    & 1.00                                     & 0.82                                  & 0.90                                    & 1.00                                     & 0.00                                  & 0.01                                    & 1.00                                     & 0.67                                  & 0.80                                    & 601                                      \\ \hline
System 4                                  & 1.00                                     & 0.49                                  & 0.66                                    & 0.84                                     & 1.00                                  & 0.91                                    & 1.00                                     & 0.37                                  & 0.54                                    & 1.00                                     & 0.96                                  & 0.98                                    & 913                                      \\ \hline
System 5                                  & 0.99                                     & 1.00                                  & 0.99                                    & 0.99                                     & 1.00                                  & 0.99                                    & 0.99                                     & 1.00                                  & 0.99                                    & 0.99                                     & 1.00                                  & 0.99                                    & 337                                      \\ \hline
System 6                                  & 1.00                                     & 0.38                                  & 0.55                                    & 1.00                                     & 0.53                                  & 0.69                                    & 1.00                                     & 0.16                                  & 0.27                                    & 1.00                                     & 0.38                                  & 0.55                                    & 721                                      \\ \hline
\multicolumn{1}{|c|}{\textbf{AVERAGES}}   & \BlackCell{1.00}                         & \BlackCell{0.34}                                  & \BlackCell{0.42}                        & \BlackCell{0.90}                         & \BlackCell{0.84}                                  & \BlackCell{0.84}                        & \BlackCell{1.00}                         & \BlackCell{0.26}                                  & \BlackCell{0.31}                        & \BlackCell{0.94}                         & \BlackCell{0.77}                                  & \BlackCell{0.81}                        &                                          \\ \hline
Core Driver 1                             & 1.00                                     & 0.46                                  & 0.63                                    & 1.00                                     & 0.90                                  & 0.95                                    & 1.00                                     & 0.38                                  & 0.55                                    & 1.00                                     & 0.61                                  & 0.76                                    & 43195                                    \\ \hline
Core Driver 2                             & 1.00                                     & 0.03                                  & 0.05                                    & 1.00                                     & 0.21                                  & 0.35                                    & 1.00                                     & 0.01                                  & 0.02                                    & 1.00                                     & 0.04                                  & 0.08                                    & 43200                                    \\ \hline
Core Driver 3                             & 1.00                                     & 0.27                                  & 0.43                                    & 1.00                                     & 0.40                                  & 0.57                                    & 1.00                                     & 0.18                                  & 0.30                                    & 1.00                                     & 0.28                                  & 0.43                                    & 43200                                    \\ \hline
Core Driver 4                             & 1.00                                     & 0.03                                  & 0.05                                    & 1.00                                     & 0.07                                  & 0.13                                    & 1.00                                     & 0.02                                  & 0.03                                    & 1.00                                     & 0.03                                  & 0.07                                    & 43200                                    \\ \hline
Core Driver 5                             & 1.00                                     & 0.22                                  & 0.36                                    & 1.00                                     & 0.41                                  & 0.58                                    & 1.00                                     & 0.15                                  & 0.25                                    & 1.00                                     & 0.23                                  & 0.38                                    & 43200                                    \\ \hline
Core Driver 6                             & 1.00                                     & 0.39                                  & 0.56                                    & 1.00                                     & 0.52                                  & 0.68                                    & 1.00                                     & 0.27                                  & 0.42                                    & 1.00                                     & 0.39                                  & 0.56                                    & 43200                                    \\ \hline
Core Driver 7                             & 1.00                                     & 0.72                                  & 0.84                                    & 1.00                                     & 0.96                                  & 0.98                                    & 1.00                                     & 0.59                                  & 0.74                                    & 1.00                                     & 0.77                                  & 0.87                                    & 43200                                    \\ \hline
Core Driver 8                             & 1.00                                     & 0.24                                  & 0.39                                    & 1.00                                     & 0.29                                  & 0.45                                    & 1.00                                     & 0.13                                  & 0.24                                    & 1.00                                     & 0.24                                  & 0.39                                    & 43200                                    \\ \hline
Core Driver 9                             & 1.00                                     & 0.35                                  & 0.52                                    & 1.00                                     & 0.56                                  & 0.72                                    & 1.00                                     & 0.30                                  & 0.46                                    & 1.00                                     & 0.40                                  & 0.58                                    & 43178                                    \\ \hline
Core Driver 10                            & 1.00                                     & 0.14                                  & 0.25                                    & 1.00                                     & 0.28                                  & 0.43                                    & 1.00                                     & 0.05                                  & 0.09                                    & 1.00                                     & 0.15                                  & 0.26                                    & 43200                                    \\ \hline
\multicolumn{1}{|c|}{\textbf{AVERAGES}}   & \BlackCell{1.00}                         & \BlackCell{0.29}                                  & \BlackCell{0.41}                        & \BlackCell{1.00}                         & \BlackCell{0.46}                                  & \BlackCell{0.58}                        & \BlackCell{1.00}                         & \BlackCell{0.21}                                  & \BlackCell{0.31}                        & \BlackCell{1.00}                         & \BlackCell{0.32}                                  & \BlackCell{0.44}                        &                                          \\ \hline
\multicolumn{1}{|c|}{\textbf{TOTAL AVERAGES}}     & \BlackCell{0.87}                 & \BlackCell{0.39}                                  & \BlackCell{0.41}                                & \BlackCell{0.77}                 & \BlackCell{0.71}                                  & \BlackCell{0.65}                                & \BlackCell{0.90}                 & \BlackCell{0.32}                                  & \BlackCell{0.33}                                & \BlackCell{0.81}                 & \BlackCell{0.63}                                  & \BlackCell{0.60}                                & 435603                                   \\ \hline
\end{tabular}
}
\caption{CapEng and User Behavior Precision, Recall, and F-measure Results} 
\label{tab:fmeasure-table-service-owner-master}
\end{table*}


==> sesd-shesd-tables-include.tex <==
\begin{table*}[H]
\begin{minipage}{\textwidth}
\input{sesd-shesd-cap-ub-fmeasure-table.tex}
\end{minipage}
\begin{minipage}{\textwidth}
\input{sesd-shesd-inj-fmeasure-table.tex}
\end{minipage}
\label{tab:fmeasure-table-injection-master}
\end{table*}

==> summary-cap-ub-table.tex <==
\begin{table*}[ht]
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|l|}
\hline
\multirow{2}{*}{}                       & \multicolumn{6}{|c|}{\textit{Alpha = 0.05 (95\% Confidence)}}                                     & \multicolumn{6}{|c|}{\textit{Alpha = 0.001 (99.9\% Confidence)}} & \multirow{2}{*}{}                                                                           \\ \cline{2-13}
                                        & \multicolumn{3}{|c|}{\textbf{S-ESD}}            & \multicolumn{3}{|c|}{\textbf{S-H-ESD}}          & \multicolumn{3}{|c|}{\textbf{S-ESD}}                 & \multicolumn{3}{|c|}{\textbf{S-H-ESD}}             & \multicolumn{1}{|c|}{\textbf{}}                                                             \\ \hline
\multicolumn{1}{|c|}{\textbf{Dataset}}  & \textit{Prec.} & \textit{Rec.} & \textit{Fmes.} & \textit{Prec.} & \textit{Rec.} & \textit{Fmes.} & \textit{Prec.}   & \textit{Rec.}   & \textit{Fmes.}  & \textit{Prec.}  & \textit{Rec.}  & \textit{Fmes.}  & \multicolumn{1}{|c|}{\textit{\begin{tabular}[c]{@{}c@{}}Total\\ Observations\end{tabular}}} \\ \hline
\multicolumn{1}{|c|}{\textbf{Averages}} & 0.90           & \textit{0.34} & 0.36           & 0.82           & 0.59          & 0.55           & 0.92             & 0.28            & 0.30            & 0.85            & 0.52           & 0.52            & \multicolumn{1}{|c|}{436,331}                                                               \\ \hline
\end{tabular}
\caption{Summary overview of Precision, Recall, and F-measure Averages for CapEng and UB Perspectives} 
\label{tab:fmeasuretableserviceowner} 
\end{table*}

==> summary-inj-table.tex <==
\begin{table*}[ht]
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|l|}
\hline
\multirow{2}{*}{}                       & \multicolumn{6}{|c|}{\textit{Alpha = 0.05 (95\% Confidence)}}                                     & \multicolumn{6}{|c|}{\textit{Alpha = 0.001 (99.9\% Confidence)}} & \multirow{2}{*}{}                                                                           \\ \cline{2-13}
                                        & \multicolumn{3}{|c|}{\textbf{S-ESD}}            & \multicolumn{3}{|c|}{\textbf{S-H-ESD}}          & \multicolumn{3}{|c|}{\textbf{S-ESD}}                 & \multicolumn{3}{|c|}{\textbf{S-H-ESD}}             & \multicolumn{1}{|c|}{\textbf{}}                                                             \\ \hline
\multicolumn{1}{|c|}{\textbf{Dataset}}  & \textit{Prec.} & \textit{Rec.} & \textit{Fmes.} & \textit{Prec.} & \textit{Rec.} & \textit{Fmes.} & \textit{Prec.}   & \textit{Rec.}   & \textit{Fmes.}  & \textit{Prec.}  & \textit{Rec.}  & \textit{Fmes.}  & \multicolumn{1}{|c|}{\textit{\begin{tabular}[c]{@{}c@{}}Total\\ Observations\end{tabular}}} \\ \hline
\multicolumn{1}{|c|}{\textbf{Averages}} & 1.00           & \textit{0.96} & 0.98           & 1.00           & 0.97          & 0.98           & 1.00             & 0.94            & 0.96            & 1.00            & 0.95           & 0.97            & \multicolumn{1}{|c|}{345,600}                                                               \\ \hline

\end{tabular}
\caption{Summary overview of Precision, Recall, and F-measure Averages Injection Perspective} 
\label{tab:fmeasuretableinjection} 
\end{table*}

==> tiejen-moore.tex <==
\subsubsection{Teijen-Moore Test} \label{sec:tmoore}

The Tietjen-Moore test \cite{tietjen_grubbs-type_1972} is a generalization of
the Grubbs' test for detecting $k$ anomalies. %In the specific case of testing

The data is first sorted from smallest to largest. Then, the following test 
statistic is computed using the $k$ largest values:

\begin{equation} 
C_{k}=\frac{\sum_{i=1}^{n-k} (x_{i}-\bar{x_{k}})^{2}}{\sum_{i=1}^{n} (x_{i}-\bar{x})^{2}} 
\end{equation} 

\noindent
where, $x_{i}$ represents the $i^{\text{th}}$ largest value in the data set. 
A critical region is then calculated by generating a normally distributed 
random sample, and calculating the test statistics for the $k$ largest values 
in the same manner as before. The two sets of test statistics are then compared 
in order to determine if the data set contains anomalies.  

The Tietjen-Moore test requires that $k$ be specified.

